CoEvoke: Evoking Multi-Agent Collaboration for Trajectory Collection

Training multi-agent collaboration requires trajectories of checking, feedback, and repair, yet task-solving rollouts may end in immediate approval or repeat unsuccessful attempts without useful correction. We introduce CoEvoke, a cross-domain framework that evokes these interactions during trajectory collection. Controlled perturbations create recoverable difficulties, while restricted reference-based guidance directs investigation. The resulting dataset contains 4,567 reconstructable trajectories over 4,130 software-engineering and reasoning tasks, linking public interactions to evidence, decisions, and task-native outcomes. Separate experiments over 2,287 same-task pairs show feedback increases of 47.72-100 percentage points across seven perturbation groups; guidance has smaller, model-dependent effects. With identical training tasks, decision-record counts, and updates, perturbation-enriched judge training improves ACPBench-Hard success from 35.38% to 42.12% (+6.73 points). SWE verifier training gains 7.60-9.40 points over interface-matched untrained references. Workflow and post-training evaluations preserve task-solving topology with unperturbed inputs and no private-reference guidance. These results support designing collection conditions to obtain corrective supervision that improves collaborative decisions with frozen solving agents.

==> table_style.tex <==
% Shared table presentation. Figures and the conference template are unchanged.
\RequirePackage{etoolbox}
\definecolor{tblInk}{HTML}{2F3F49}
\definecolor{tblRule}{HTML}{52616C}
\definecolor{tblHead}{HTML}{DFE1E9}
\definecolor{tblSection}{HTML}{D4D9E2}
\definecolor{tblStripe}{HTML}{F2F3F5}
\definecolor{tblSummary}{HTML}{E7ECEB}
\definecolor{tblRise}{HTML}{965C48}
\definecolor{tblFall}{HTML}{3F7982}
\definecolor{tblTokenBlue}{HTML}{5B88A6}
\definecolor{tblNeutral}{HTML}{737D84}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{N}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\tblhead}[1]{\textcolor{tblInk}{\textbf{#1}}}
% Padding belongs inside each multiline cell. A taller array strut alone has
% no effect when the stack is already taller than that strut.
% Use the current font's normal baseline distance, so adjacent two-line
% headings align even when their letters have different heights/depths.
% Preserve colortbl state without a nested colored tabular.
\makeatletter
\iflatexml
\newcommand{\tblstack}[1]{\shortstack[c]{#1}}
\else
\newcommand{\tblstack}[1]{\ensuremath{\vcenter{%
  \kern2.4pt
  \hbox{\vbox{\normalbaselines
    \CT@start\ialign{\hfil\strut##\hfil\cr#1\crcr}\CT@end}}%
  \kern2.4pt}}}
\fi
\makeatother
\newcommand{\tblkey}[1]{\textbf{#1}}
\renewcommand{\best}[1]{\textbf{#1}}
\renewcommand{\second}[1]{\underline{#1}}
\newcommand{\gain}[1]{\textcolor{tblRise}{\ensuremath{\uparrow}\,#1}}
\newcommand{\loss}[1]{\textcolor{tblFall}{\ensuremath{\downarrow}\,#1}}
\newcommand{\tokendrop}[1]{\textcolor{tblTokenBlue}{\ensuremath{\downarrow}\,#1}}
\newcommand{\same}[1]{\textcolor{tblNeutral}{#1}}
\newcommand{\tablepresentation}{%
  \arrayrulecolor{tblRule}%
  \setlength{\heavyrulewidth}{.75pt}%
  \setlength{\lightrulewidth}{.38pt}%
  \setlength{\cmidrulewidth}{.3pt}%
  % Put breathing room inside the colored cells, not between fill and rules.
  \setlength{\aboverulesep}{0pt}%
  \setlength{\belowrulesep}{0pt}%
  \setlength{\cmidrulesep}{0pt}%
  \setlength{\extrarowheight}{1.1pt}%
  \setlength{\belowcaptionskip}{4pt}%
  \renewcommand{\arraystretch}{1.05}}
\AtBeginEnvironment{table}{\tablepresentation}
\AtEndEnvironment{table}{\arrayrulecolor{black}}

